Toward Reliable Models for Authenticating Multimedia Content: Detecting Resampling Artifacts With Bayesian Neural Networks

In multimedia forensics, learning-based methods provide state-of-the-art performance in determining origin and authenticity of images and videos. However, most existing methods are challenged by out-of-distribution data, i.e., with characteristics that are not covered in the training set. This makes it difficult to know when to trust a model, particularly for practitioners with limited technical background. In this work, we make a first step toward redesigning forensic algorithms with a strong focus on reliability. To this end, we propose to use Bayesian neural networks (BNN), which combine the power of deep neural networks with the rigorous probabilistic formulation of a Bayesian framework. Instead of providing a point estimate like standard neural networks, BNNs provide distributions that express both the estimate and also an uncertainty range. We demonstrate the usefulness of this framework on a classical forensic task: resampling detection. The BNN yields state-of-the-art detection performance, plus excellent capabilities for detecting out-of-distribution samples. This is demonstrated for three pathologic issues in resampling detection, namely unseen resampling factors, unseen JPEG compression, and unseen resampling algorithms. We hope that this proposal spurs further research toward reliability in multimedia forensics.

==> old_intro_stuff.tex <==
% 
% % 
% % %Early methods perform this validation with an explicit
% % %model on image formation, e.g., by checking the consistency of
% % %lighting~{\color{red}{REF}}, fixed pattern sensor noise~{\color{red}{REF}}, or
% % %JPEG compression artifacts~{\color{red}{REF}}. In order to cope with
% % %increasingly complex image operator chains, e.g., in images from smartphone
% % %cameras or downloaded from social media sites, recent approaches are oftentimes
% % %learning-based. Notable examples include learning of blind noise
% % %statistics~\cite{cozzolino2019noiseprint}, relations between EXIF tags and the
% % %image statistics~{\color{red}{REF HUH}}, or artifacts of commonly used
% % %operators~{\color{red}{REF STAMM}}.
% % 
% % Besides many remarkable research results, it is still an open problem to
% % successfully transfer these methods into practice.  For example, in law
% % enforcement, which is traditionally an important potential user community, a
% % commonly raised concern is \emph{whether and to which extend we can trust the
% % result of a forensic method}. This is also an important question to other user
% % groups such as journalists, who oftentimes have to assess the authenticity of
% % images or videos with little context knowledge on the provenance.
% % 
% % This scepticism can be better understood from the perspective of the analyst:
% % here, each case is unique. For example, when searching for statistical
% % artifacts of image tampering, it is simply not possible to enumerate the
% % possible combinations of camera hardware artifacts, camera postprocessing
% % pipelines, and the possibilities of further processing by social networks.\blnote{Der Zusammenhang von statistischen Artefakten zum Aufzählen aller Verarbeitungsschritte ist nicht offensichtlich.}
% % Hence, in an actual case, it is likely that an analyst has to work with tools
% % that have never been tested under the specific hardware and software
% % combination. Yet, the analyst has to be able to defend her assessment whether
% % an image or video is authentic. This puts the analyst in a difficult predicament:
% % model-based methods typically provide specific assumptions that allow to check
% % the validity of an algorithmic result, but their baseline performance is
% % limited in cases where the image or video has undergone complex processing.
% % Hence, the \emph{a priori} probability of error is considerable.
% % Learning-based methods exhibit a much stronger baseline performance on such
% % complex processing chains. This makes learning-based methods in principle more
% % suitable for an investigator. However, their assumptions are significantly more
% % difficult to validate, particularly for an analyst with limited technical
% % background. Even worse, learning-based frameworks have the tendency to silently
% % fail with overly confident decisions. This particularly happens in cases when
% % the testing distribution is different from the training distribution, commonly
% % referred to as \emph{training-testing mismatch} \cite{cozzolino2018forensicTransfer}{\color{red}{REF REF}}.\blnote{Einige Arbeiten zu out-of-distribution detection zitieren auch https://arxiv.org/abs/1606.06565 wo das Problem ``distributional shift'' genannt wird.}
% % In forensic applications, we argue that we can already make great progress by
% % \emph{detecting} a training-testing mismatch in the data, in order to let the
% % analyst know when the classifier is not confident in its decision.\blnote{Standard CNN is confident but should not be.}
% % 
% % %This predicament is not easy to solve. We argue that new design paradigms are
% % %required to support the adoption of forensic algorithms by practitioners.
% % %Towards this goal, \emph{we make the assumption that such a solution has to be
% % %learning-based} to preserve the flexibility and strong empirical performance of
% % %a data-driven framework.
% 
% Towards this goal, we propose to formulate the forensic learning task within a
% Bayesian framework. This formalism allows to learn a data distribution, and to
% perform inference between the learned distribution and the input data. This
% framework provides not only a classifier decision, but also an uncertainty in the
% decision. More specifically, this work contains three contributions:
% \begin{enumerate}
% \item We propose Bayesian Neural Networks for modeling uncertainty in image
% forensics. To our knowledge, this is the first time that Bayesian networks are
% used in image forensics.
% \item We show a proof-of-concept binary classification application on the popular forensic task of
% resampling detection. The network achieves state-of-the-art performance, with
% the added benefit of detecting out-of-distribution samples.
% \item We compare the Bayesian network's predictive uncertainty to confidence derived from softmax statistics~\cite{hendrycks17softmaxStatisticsBaseline}.
% \end{enumerate}
% 
% This paper is organized as follows. In Section~\ref{sec:related_work} we describe related work regarding the image forensics topic as well as the application of Bayesian methods for neural networks in related research fields. Section~\ref{sec:methods} introduces the basic concepts of the Bayesian formalism for convolutional neural networks (CNNs) and variational approximation. In Section~\ref{sec:experiments} we discuss empirical results on the binary classification problem of resampling detection. We conclude with a brief summary and outlook in Section~\ref{sec:conclusion}.  

%When a neural network architecture

%Bayesian networks feature a theoretical sound framework

%Researchers have developed a broad set of tools to identify and localize image tampering. These tools target different application scenarios and groups of potential users.
%Existing tools can be split into model-based and learning-based approaches.

% Analytical model-based approaches
% Note that this paragraph is inspired by Christian's project description on the RTG proposal
%Traditional methods are based on analytical models, which make explicit assumptions of input signals' properties, either in feature or frequency domain. For example, Fridrich and Kodovský model the statistics of natural images, and identify potential tampering from anomalies in noise or compression patterns~\cite{fridrich2012richModels}. Similar techniques have been proposed for modeling traces of image formation or scene properties~\cite{ng06passiveBlindImageForensics}. Since there is an underlying mathematical model, mandatory and boundary conditions can be explicitly stated.
% If we want to be more specific regarding model-based techniques targeting traces of image formation, include references to lens distortion, camera response function, demosaicing.

% Challenges for model-based techniques
%Many model-based forensic methods, however, are based on assumptions that are very restrictive and limit the applicability of these methods in practice. When no prior knowledge about the image under analysis is available, it is far from clear whether or not that image satisfies these model assumptions, and which forensic methods can safely be employed on that image.
%Recent trends make it even harder to place or verify assumptions on an image. These trends include a shift from traditional image formation to computational imaging, the increasing development of digital image processing tools, and the distribution of images over social media.

% Shift towards learning-based methods
%With recent advances in applied machine learning, the digital forensics community's focus turned from model-based to learning-based methods. Especially end-to-end learning methods based on deep neural networks have gained high popularity. Using deep neural networks, no explicit assumptions have to be made. Instead the network learns patterns from a set of training examples, leading to a more generic approach, enabling to learn powerful representations.

% Not sure if this paragraph should be moved to the related work section
%These statistical machine and deep learning approaches fit a statistical model to a high-dimensional feature space. The model aims to faithfully represent a ground truth distribution for a given task, based on data samples used to train the model. Therefore it is crucial to use training data which is representative for a specific task. However in typical real-world applications the ground truth distribution is unknown and the knowledge whether the training data is representative, is not trivial. Therefore the training data is based on assumptions about the ground truth. This can lead to inaccuracies between the learned and the ground truth distribution. These differences are regions where out-of-distribution examples can be found. Standard neural network models are unable to express predictive uncertainty, and tend to overconfident predictions in such regions.

% Loose track of assumptions, boundary conditions, required for forensic analysis in legal context
%Despite outperforming model-based techniques on many tasks, methods based on deep learning also raised serious concerns regarding their ability to generalize to examples not seen during training. Since no boundary conditions can be stated explicitly, failure cases are difficult to anticipate. This lack of reliability may hinder potential users, \eg, law enforcement and forensic analysts in a legal context, to base their decisions on such tools.

% Restore some trust in machine learning with our work
%To this end, we aim to restore trust into learning-based methods by providing the analyst with an additional uncertainty estimate that can act as a metric of prediction reliability. The uncertainty estimate warns the forensic analyst about unfamiliar patterns and potential failure cases. We demonstrate how Bayesian neural networks replace standard neural networks for the task of detecting resampling artifacts, but note that Bayesian methods are applicable to any task.

%{\color{blue}{Wir haben zwei Vorteile: 1. wir sind nicht over-confident - wir sind {\"a}hnlich zu generalisiertem Dropout, 2. wir haben ein uncertainty estimate}}

%{\color{blue}{Such a training-testing mismatch has many facets in machine learning research. For example, transfer learning aims to close the mismatch by an explicit postprocessing step to reuse a pre-trained network on a new data distribution {\color{red}{REF REF}}. Another application are adversarial examples, which exploit the training-testing mismatch to purposedly misguide classifiers {\color{red}{REF REF}}.}}

%{\color{red}{Considerations on robustness: Liu/Kirchner: Ganzer Absatz darueber dass bicubische Interpolation Dinge deutlich schlechter macht. Vorgeschlagener Fix: Bicubische Interpolation in Trainingsdaten aufnehmen, aber das hat dann bilineare verschlechtert. Deep Fake-Generalisierung ueberlegen. Open-Set Generalisierung: Netzwerke oft auf 25 Kameras trainiert ($\rightarrow$ Patrick fragen), bisschen schwierig auf Open-Set zu gehen. ICLR paper von Liang, Srikant, Li: ``Enhancing the reliability of out-of-distribution image detection in neural networks: machen 2 tricks: faktor im softmax, gradienten-trick, unser Ansatz ist dagegen ein komplett bayesisches Netzwerk, was vor gericht viel besser ist. Paper zu Calibration Curves: Guo, Pleiss, (..), Weinberger: ICML-Paper, ``On Calibration of Modern Neural Networks''. ``Kalibriert'' Wahrscheinlichkeiten, weil ansonsten Wahrscheinlichkeiten aus NN nicht mit unserem Verstaendnis uebereinstimmen, und auch mathematisch sinnlos sind.}}

%{\color{red}{Outlook or so: advantage 1) of Bayesian networks is that it is not so prone to overfitting. This may be particularly useful for deepFakes. Aber nachteil: problem muss ueber priors modelliert werden.}}

%{\color{red}{Mention priors; in erstem Versuch ist Gauss'sche Prior doch gar nicht so schlecht, das kann man problemabh{\"a}ngig dann noch verbessern in future work.}}

%{\color{red}{trainierbarkeit, bzw. wie haben wir netz initialisiert, 2x so viele parameter sind halt schwieriger.}}

%
% Previous draft for introduction
%
%The determination of the authenticity of an image or video is an essential part of digital image forensics. Therefore the examination of affine linear transformations, like scaling or rotation, is of particular interest, since image manipulations almost always involve such transformations to align spliced content to fit into an image. Hence the analysis of resampled signals is a vital, and over the last decades well-studied element in digital image forensics. Traditional methods are based upon analytical models (some citations). These contain underlying mathematical models, which make explicit assumptions of input signals properties, either in feature or frequency domain. The properties can be exploited, and traces emerged from interpolation dependencies, analytically derived.
%
%(Examples for analytical model based methods.)
%over the last recent years the transition towards data driven approaches happened.
%Using deep neural network based end-to-end learning methods, no explicit assumptions have to be made. Instead the network learns patterns from a set of training samples, leading to a more generic approach, enabling to learn powerful representations. 
%
%But with the increasing development in digital image processing tools on the one hand and problems like social media, which perform high compression on uploading an image which can be interpreted as some kind of laundering operation, partly destroying resampling traces, on the other hand. With the emergence of deep learning based approaches, these also have become popular in the digital image forensics research field.
%
%These data driven approaches 
%
%
%over the last recent years the transition towards data driven approaches happened. Using deep neural network based end-to-end learning methods, no explicit assumptions have to be made. Instead the network learns patterns from a set of training samples, leading to a more generic approach. These neural network approaches lead to more generic approaches, enabling the learning of powerful representations  
%
%
%Since there is an underlying mathematical model, continuity and consistency assumption are made, either regarding input pixel distribution or the pixel statistics.
% Since there is an underlying mathematical model, mandatory and boundary conditions can be explicitly stated.
% But with the increasing development digital image processing tools on the one hand and problems like social media, which perform high compression on uploading an image what can be seen as laundering operation destroying traces of potential image tampering, on the other hand. With the emergence of deep learning based approaches, these become also popular in the research area of digital image forensics. 

% In the last recent years, data driven approaches, had a significant impact on a wide variety of different topics. Especially, end-to-end learning methods based on deep neural networks, or deep learning based models have gained high popularity. These methods fit a statistical model to a high dimensional feature space

% learn powerful representations which can map high dimensional input data to a discrete finite set of observations, given a set of training samples. These models aim to faithfully represent a ground truth distribution of a given task, based on data samples used to train the model. Therefore it is crucial to use training data which is representative for a specific task. However 

% These statistical machine and deep learning approaches fit a statistical model to a high-dimensional feature space. The model aims to faithfully represent a ground truth distribution of a given task, based on data samples used to train the model. Therefore it is crucial to use training data which is representative for a specific task. However in typical real-world applications the ground truth distribution is unknown and the knowledge whether the training data is representative, is not trivial. Therefore the training data is based on assumptions about the ground truth. This can lead to inaccuracies between the learned and the ground truth distribution. These differences are regions where out-of-distribution examples can be found. Standard neural network models are unable at expressing predictive uncertainty, and tend to overconfident predictions in such regions.

% In a real-world setting, passive forgery detection needs to work in the absence of prior knowledge about the original image, \ie, the origin and processing history of an image under analysis are usually unknown. Here it is crucial to know when the image under analysis does not match to the training distribution, to prevent erroneous conclusions.
% % Machine learning generalizes well to test data that is sampled from the same distribution as the training data. When we apply machine learning-based classifiers, we implicitly assume that the test sample matches the training distribution.
% % Some people call this distributional shift

% In this work we describe a bayesian approach towards neural networks for digital image forensics task, by learning a probability distribution on the weights instead of point estimates. We show how based on this approach the model is able to express predictive uncertainty, and how this uncertainty can act as a metric of prediction reliability for forgery detection.



